Countering the Path Explosion Problem in the Symbolic Execution of Hardware Designs

Symbolic execution is a powerful verification tool for hardware designs, but suffers from the path explosion problem. We introduce a new approach, piecewise composition, which leverages the modular structure of hardware to transfer the work of path exploration to SMT solvers. We present a symbolic execution engine implementing the technique. The engine operates directly over register transfer level (RTL) Verilog designs without requiring translation to a netlist or software simulation. In our evaluation, piecewise composition reduces the number of paths explored by an order of magnitude and reduces the runtime by 97%. Using 84 properties from the literature we find assertion violations in 5 open-source designs including an SoC and CPU.

==> dacreviews.tex <==
\section{DAC Reviews}
\cks{From DAC reviews:}
\begin{itemize}
\item read Kolbl DAC 2001~\cite{kolbl2001symbolic} paper. How does this compare and contrast?
\item what is the memory usage? We have to store symbolic state and path
  conditions of all paths in all blocks.
\item Done. Change figure 1 to be using two always blocks instead of two if
  statements
\item Compare to state of the art MC or SE tool. RTLContest is concolic
  execution, not symbolic execution, not a fair comparison.
\item How common is it for always blocks to be independent? (We didn't
  do a good job conveying the point that all always blocks are
  independent for legal designs)
\item More clear exposition is needed to establish the novelty of the
  approach and why it works. Explain the promise of this approach over
  \cite{knox,meng2021rtlcontest,mukherjee2015hardware} 
\item Add running example, walk through as we explain the technique,
  show the queries to the SMT solver.
\item Evaluation should be in comparison to \cite{knox,meng2021rtlcontest,mukherjee2015hardware} if
  possible.
\end{itemize}



==> design-old.tex <==
% 1. Preprocessing
% 2. Symbolic Execution
% 2.a. Building/Defining semantics for symbolic execution
% 2.b. Building the tree/using the constraint solver
% 2.c. Challenges (in no particular order)
% 2.c.i. continuous assignments (introduce the 2 queues example; use email
% to/from Kaki)
% 2.c.ii. ITE vs branching (this might get first mention in (2a))
% 2.c.iii. nonblocking assignments/always blocks
% 2.c.iv. multiple clock cycles
% 2.c.v. dependencies between modules/hierarchical modules (continue the 2 queues example)
% 3. Optimizations/Opportunities in HW 
% 3.a. optimization across always blocks -- SExplore once and merge
% 3.b. COI analysis (I think COI refers to gate-level analysis
% specifically. We need another name maybe?)
% 3.c. redundant submodules -- SExplore once and merge
% 4. Assertion Violations (maybe this now goes between 2b and 2c)
%% Not sure where this goes, but:
% Search
%% CFG keeps track of where we've been
%% How to decide where to search next
%% Optimization of not re-searching a submodule
%%% Describe first conceptually, using the formal notation introduced to
% describe SE; then give toy example. If there are particulars of how its
% implemented that are interesting, they go in impelementation section.


Sylvia works in two phases as shown in Figure~\ref{fig:overview}: Preprocessing
and Symbolic Execution. We start with an overview of Sylvia and then delve into
the details, including a description of how Sylvia leverages the common
characteristics of hardware designs to optimize search.

\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth,trim=.5in 3.6in .5in 0in,
    clip]{figures/overview}
  \caption{An overview of Sylvia's design.}
  \label{fig:overview}
\end{figure}

\textbf{Preprocessing}. As a first step, the Verilog RTL is parsed to build an abstract
syntax tree (AST). Sylvia then performs a single AST traversal to build a flattened
representation of the design's decision points, a bitstring that we call the
\emph{pathcode}. This is a key part of the interface between the AST and
execution engine used to guide exploration and inform which branches are to be
explored in a given run of symbolic execution. This phase also involves a
preliminary dependency analysis that discovers the ordering of the dependent submodules
to be symbolically executed. 

\textbf{Symbolic Execution}. \cks{revisit} The core phase of the symbolic execution engine is powered by AST traversals where each individual tree traversal corresponds to a new path through the design. This involves interpreting Verilog AST nodes as instructions to be executed and implementing a faithful symbolic semantics of Verilog in Python. The parallelism and hierarchical structure of hardware designs present unique challenges to development of a software-style symbolic execution engine. In section 4.2.5-4.2.8 we go into detail about each one and provide details on our solution. 

As the exploration progresses, Sylvia pushes constraints to an SMT solver, Z3 \cite{de2008z3}, keeping track of what conditions have brought us down a particular path. At the end of each run of the engine, we can solve for these constraints and use Sylvia to find security assertion violations.

 \textbf{Optimizations}. Sylvia leverages the modular nature and the structural and behavioral parallelism inherent to many RTL designs to mitigate the path explosion problem and reduce
 the complexity of queries to the constraint solver. Optimization passes perform
 analyses to identify sets of execution states that can be merged and to
 restrict the search to areas of the design pertinent to the given security assertions.

 

\subsection{Preprocessing}
In the first phase, Sylvia builds the data structures necessary for symbolic execution. At the end of preprocessing Sylvia has an abstract
syntax tree (AST) representation of the design, an accounting of the conditional
dataflow points in the design, and a dependency graph of modules in the design showing
the dataflow relationship between modules in which one module reads a register
or wire written to by another module.

\begin{figure}[t]
  \centering
  \adjustbox{trim={.01\width} {.00\height} {0.01\width} {.00\height},clip}%
 % { \includegraphics[width=\columnwidth, keepaspectratio,height=7cm,
  % width=9cm]{figures/queue_ast}}
   { \includegraphics[width=.6\columnwidth, keepaspectratio]{figures/queue_ast}}
  \caption{Snippet of Queue Module AST.}
  \label{fig:ast}
\end{figure}

\subsubsection{The Abstract Syntax Tree (AST)}
An abstract syntax of a language keeps the core arithmetic expressions, boolean expressions,
and commands that make up the language, while dropping the written syntax,
such as the semicolon, that is used for reading and writing code. The AST of a
Verilog design represents the
complete design as a tree, with the root and internal nodes corresponding to
commands and operators in the abstract syntax of Verilog, and leaf nodes corresponding to the signals, registers,
ports, and literal values in the design. Once built, the AST serves as the
authoritative representation of the design; Sylvia symbolically executes the design
by traversing the AST. Figure~\ref{fig:ast} shows a snippet of the AST
corresponding to the queue module in Figure~\ref{lst:queuemodule}. The dotted lines mean that additional child Nodes would be 
expected to stem from that particular parent Node but are elided for the purpose of brevity.  



\subsubsection{Conditional Dataflow}
In the synthesizable subset of Verilog accepted by Sylvia, the language constructs that represent decision points in how data flows through
the design are $\texttt{if}\ldots\texttt{else}$, including nested $\texttt{else if}$s, ternary
if-then-else ($\texttt{?\ldots:}$), $\texttt{case}$, and $\texttt{for}$. \cks{maybe we
  need a small table that is: exact syntax of each construct; number of
  branches.} The $\texttt{if}$ statements always yield two
branches ($\texttt{else if}$ statements are treated as nested $\texttt{if}$s).
The number of branches in a $\texttt{case}$ statement is determined by the
number of alternatives, i.e., the number of possible cases. The number of
branches in  $\texttt{for}$
loop is determined statically by the initial state and condition of the loop. 

Sylvia does a preliminary traversal of the AST to assess the path complexity of the design. An
accounting of the decision points in the design is taken and an upper
bound on the number of possible paths is calculated. The \emph{pathcode} is also
built. The pathcode is a bitstring with one bit allocated for boolean condition to be evaluated across as part of a decision
point in the design.  An $\texttt{if}$ is a decision point with two branches, where one condition is evaluated, and gets one 
bit in the pathcode. A $\texttt{case}$ statement is a decision point with the number of branches 
determined by the number of alternatives. A $\texttt{case}$ statement with N alternatives would be allocated N bits -- one bit for each possible condition evaluated during the exploration of the $\texttt{case}$ statement. 

Symbolic execution of a hardware design treats
the data flow decision points in the design -- those language constructs that
can be synthesized into MUXes -- as control flow execution points. In each
run/iteration, Sylvia follows a single path of data flow. For example, an
$\texttt{if}\ldots\texttt{else}$ statement would yield two paths to follow, one
in which the condition is assumed to be true and one in which it is assumed to
be false. \kar{I moved this from the background, maybe can be weaved in better, but I think its helpful}

\begin{figure}[t]
  \centering
  \adjustbox{trim={.01\width} {.00\height} {0.01\width} {.00\height},clip}%
 % { \includegraphics[width=\columnwidth, keepaspectratio,height=7cm,
  % width=9cm]{figures/queue_ast}}
   { \includegraphics[width=.8\columnwidth, keepaspectratio]{figures/dependencies_modules}}
  \caption{Illustration of dependencies between modules}
  \label{fig:dependencies_modules}
\end{figure}


\subsubsection{Preliminary Dependency Analysis}
The hierarchical and modular nature of hardware means that submodules are
operating in parallel and the output signals of some modules become
the input to other modules. Before symbolic execution can begin, Sylvia computes
the dependency graph of modules. Each module of the design is represented as a
node in the graph, and directed edges between nodes represent a read--write
dependence. From this graph, an order of execution of modules in the
design can be computed. Figure~\ref{fig:dependencies_modules} shows a simple
example, in which module A has an input that depends on module B's
output, and B has an input that depends on C's output. Sylvia will explore the modules in the necessary order to resolve the
dependency: C followed by B, and then B followed by A. On the other hand, independent modules
for which there is no path from one to the other in the dependency graph,
present an opportunity for optimization. We discuss the optimization in
Section~\ref{sec:redundantmodules}.

\subsection{Symbolic Execution}
\kar{I think we should maybe have a different title for this? Or a different title for the section in the background, since they are both called Symbolic Execution}
The execution state of Sylvia is defined by the AST, pathcode, symbolic store,
and path condition. Symbolic execution proceeds by traversing the AST, using the
pathcode to guide the traversal. As execution progresses, Sylvia interprets each language construct in the
AST using an extended semantics of Verilog that includes a notion of symbols
to update the symbolic store and path condition. %\cks{this is a long sentence!} %\kar{I split it}!

If a security assertion is violated by any traversal, a satisfying solution to
the associated path condition will produce concrete values that can be used to
drive concrete execution (either in simulation or on a synthesized design) to
the violating state.

\subsubsection{The Symbolic Store}
In traditional software-style symbolic execution, engines developed for software programs will 
maintain a symbolic store, or a mapping between program variables and symbolic expressions. 
In Sylvia, we maintain mappings between the signals, registers, and ports of the hardware design
and their respective symbolic expressions. At the beginning of each clock cycle, all input ports in the top level module will
be given fresh symbols in the symbolic store. As execution proceeds and different areas of the design
are explored, the values held in the symbolic store will be updated according to the semantics of each
Verilog statement that gets symbolically executed, ensuring clock-cycle accuracy at the end of every cycle. 

\subsubsection{Defining a Symbolic Verilog Semantics}

We define an extended semantics to Verilog that introduces the notion
of symbolic values. In this paper we will use $\alpha$, $\beta$, and $\gamma$ to
represent symbols, although in practice each symbol is a unique alphanumeric
string. Symbols are used to replace literal input values to a design. In the
queue module, for example, the $\texttt{write\_data}$ input net can be
initialized with the symbolic value $\alpha$.

Symbolic execution proceeds by traversing the AST. At each node of the AST,
Sylvia uses the extended semantics of Verilog to interpret the Verilog construct
in the presence of symbols. As a replacement to literal values, symbols may
appear on the right-hand side of assignment expressions or in the condition of a
decision point. Nets ($\texttt{wire}$s) and variables ($\texttt{reg}$s) may hold
symbolic values at any point of execution.

\textbf{Declarations}. The declaration of $\texttt{reg}$s (state-holding
variables), and input $\texttt{wire}$s can be made symbolic. In this case the
interpreted variable is given a fresh symbolic value in the symbolic
store. 

\textbf{If and Case}. If the bit in the \textit{pathcode} corresponding to the particular 
$\texttt{if}$ or $\texttt{case}$ condition is set to 1, that means the condition is being
evaluated as $\texttt{True}$. This conditional expression, which is either an identifier or some 
combination of operators over identifiers and literals, is parsed and interpreted such that all
identifiers are replaced by their corresponding symbolic expressions held in the symbolic store.
Once the condition is made symbolic, we attempt to simplify it, add it to the path condition, and begin exploration
of the statement in the then block. If the bit in the  \textit{pathcode} were set to 0, we would do the same, 
but with the negation of the condition. 

\textbf{Blocking Assignment}. Visiting blocking assignment statements results in updates to the symbolic store. 
When some $\texttt{lhs}$ gets assigned some $\texttt{rhs}$, the entry in the symbolic store for the $\texttt{lhs}$ 
is immediately overwritten to hold the symbolic expression residing in the symbolic store for the $\texttt{rhs}$.

\textbf{Non-blocking Assignment}. Non-blocking assignments similarly result in updates to the symbolic store.
However, several non-blocking assignments can take place in parallel within the same clock cycle. \kar{I'm not totally sure what to write for these little paragraphs without accidentally just explaining the challenge/solution}


%%\cks{cut}
%% Sylvia is a dynamic symbolic execution that falls under the umbrella of execution-generated testing. This execution is driven by the interpretation of Verilog AST nodes as instructions to be executed, and as such, we needed to implement a faithful \textit{symbolic} Verilog semantics in Python. In some cases this was straightforward, such as interpreting a Register Declaration AST node as an instruction that should declare or initialize a symbolic variable with the same name and width in the symbolic variable store accordingly. However, in many cases, this was not as straightforward and was not comparable to translating one programming language to another because of the parallelism and hierarchy inherent in hardware. In the challenges section, we will discuss the ways we handled unique hardware constructs in software and then in the optimizations sections, we will provide details about how we were even able to leverage these features for performance gain.

%% CFG keeps track of where we've been
%% How to decide where to search next
%% Optimization of not re-searching a submodule

\begin{figure}[t]
  \centering
  \adjustbox{trim={.00\width} {.00\height} {0.00\width} {.00\height},clip}%
 % { \includegraphics[width=\columnwidth, keepaspectratio,height=7cm,
  % width=9cm]{figures/queue_ast}}
   { \includegraphics[width=.8\columnwidth, keepaspectratio]{figures/traversals}}
  \caption{AST Traversals/Updating Symbolic Store}
  \label{fig:traversals}
\end{figure}

\subsubsection{Traversing the AST}

Symbolic execution proceeds by traversing the AST. In each traversal Sylvia
visits a subset of the nodes in the AST, corresponding to one path through the
design. Sylvia uses the pathcode built during preprocessing to keep track of
which nodes in the AST to visit during a particular traversal. Recall that each
bit in the pathcode corresponds to one branch point in the design. If the bit
is set to 1, Sylvia will follow the branch, otherwise it will not. 

%% \cks{shortened text a bit}
%% AST traversals are the main mechanism by which Sylvia performs the symbolic execution of the hardware design. The high-level idea is that with each traversal we are visiting a subset of the constructs within the AST. This subset is able to reconstruct one particular control flow path through the hardware design. To get a particular subset of constructs to explore we use the \textit{\textit{pathcode}}, which is just a flattened representation of the CFG for the design. This bitstring will inform which controlflow structures to traverse and which to ignore. 

%% encodes the particular path to be explored by the symbolic execution engine. One
%% bit is allocated for each possible branch. 

%% So, consider the design in figure X, which is a snippet from an adapted implementation of the two queues schematic presented in \cite{Chatterjee2021TwoQueues}. This particular snippet just shows the code for a single queue. It has two unnested if-statements in the always block. The \textit{pathcode} being set to \textit{00} would direct Sylvia to execute the else-blocks at each juncture, which in the case of this example, are empty. Each time it reaches one of the branching statements, the bit being set to 0 would drive execution down the ``false'' branch. Alternatively, a \textit{pathcode} instance of \textit{01} would lead Sylvia down the else-block at the first juncture, but at the second branching statement, it would enter the then-block and execute the assignment on line 20. 

Every traversal begins from the top level module and proceeds downward. As
execution proceeds Sylvia updates the symbolic store according to the extended
semantics of Verilog. Figure \ref{fig:traversals} illustrates this flow where we have a line of 
Verilog RTL being built into its corresponding AST representation, and symbolically executed,
resulting in an appropriate update to the symbolic store.

\begin{figure}[t]
  \centering
  \adjustbox{trim={.01\width} {.00\height} {0.01\width} {.00\height},clip}%
 % { \includegraphics[width=\columnwidth, keepaspectratio,height=7cm,
  % width=9cm]{figures/queue_ast}}
   { \includegraphics[width=.8\columnwidth, keepaspectratio]{figures/smt_queries}}
  \caption{SMT Queries}
  \label{fig:smt_queries}
\end{figure}

\subsubsection{Updating the Path Condition} Each traversal begins with the path
condition set to $\texttt{True}$. At each branch point in the AST
traversal, Sylvia updates the path condition by pushing the constraints of the
decision point to an instance of an satisfiability modulo theories (SMT) solver
(e.g.,~\cite{de2008z3}). Before proceeding down a branch, Sylvia checks whether
the path condition is satisfiable. If it is, Sylvia continues. If it is not, the
particular path is not feasible, Sylvia halts the traversal, and proceeds to the
next path. At the end of a traversal, the satisfying solution to the path
condition will provide concrete values to all input nets and variables that
were initialized to be symbolic. If the path explored was one where an
assertion violation was encountered, these concrete values are guaranteed to
drive execution to the assertion-violating state. Figure \ref{fig:smt_queries} illustrates this flow where we
have an exploration of the design resulting in an update to the path condition, which can be 
sent to the SMT solver to produce assertion violations.

\subsubsection{Continuous Assignments}
\label{sec:continuousassignments}
Continuous assignments are used to model combinational logic in Verilog and are denoted
using the keyword \texttt{assign}. For example, lines 24-26 in
Figure~\ref{lst:queuemodule} are all continuous assignments. In a continuous
assignment, anytime any of the signals on the right-hand side of the assignment
change value, the right-hand side is re-evaluated, and the left-hand side wire
is updated. This can be a problem for Sylvia: if the variables on the right-hand
side of a continuous assignment change after Sylvia has already visited the
assignment, Sylvia would fail to note the new
value for the left-hand side. We destruct the continuous-assignment problem into
four cases, and consider each one in turn, using snippets of Verilog to explain
the problem and our solution. 
 
 \begin{enumerate}
 
\item \textbf{Case 1}. $\mathtt{assign} ~~\mathrm{read\_data} = \mathrm{input\_signal};$
	
	When an input\_signal, for example, is coming from a sensor, it can change at
  any time before, during, or after a clock cycle. Sylvia makes the assumption
  that all input signals to the top-level module remain fixed for the duration
  of a clock cycle. These top-level input signals get a fresh
  symbolic value at the start of each clock cycle, and keep that symbolic value
  for the duration of the clock cycle.%%  In other words,  input\_signal gets a fresh symbolic value
  %% at the start of a clock cycle and it keeps that symbolic value for the
  %% duration of the clock cycle unless written to via some assignment statement in
  %% the Verilog code.
%   \cks{I changed this b/c I don't think input\_signal would
%-    get a fresh symbolic value unless it were a top-level input, in which case
%-    it can't be written to. inputs to one module that are the output of some
%-    other module instead get the value determined by that other module at each
%-    clock cycle, not a fresh symbolic value. I also don't think Sylvia assumes
%-    that all inputs remain fixed for the clock cycle -- Sylvia only makes that
%-    assumption for top-level inputs. The second pass that is described below is
%-    there to handle the case where non-top-level-inputs change during a clock
%-    cycle. Kaki, will you make sure my reasoning is correct?}
% ^ this is correct
	
	
\item \textbf{Case 2}. $\mathtt{assign} ~~\mathrm{read\_data} = \mathrm{content}[31:0];$ 
	
	The right-hand side, content, is a register and its value changes only at
  clock cycle boundaries. The symbolic expression associated with
  $\mathtt{assign}$ has to be re-evaluated at the end of the clock cycle to
  catch any changes to content within that clock cycle. Sylvia re-evaluates
  left-hand side of any continuous assignment one time at the end of the clock
  cycle. The new value will
  reflect any changes in the values of the right-hand side expression. 
%  \cks{this
%-    was referring to other signals not in this example (e.g., writedata). I
%-    rewrote it to use the signals in this example. Kaki, will you fact check it?}
% KAR: looks good to me!
	
	
\item \textbf{Case 2a}. $\mathtt{assign} ~~\mathrm{read\_data2} = \mathrm{some\_content}[31:0];$\\
\-\qquad\qquad$\mathtt{assign} ~~\mathrm{read\_data} = \mathrm{read\_data2} ~\&~ \mathrm{content};$
	
A variant of Case 2 requires additional consideration.	In this Case, at the end
of the clock cycle, Sylvia has to make sure to re-evaluate write\_data2 before
re-evaluating write\_data. Sylvia does the dependency analysis between
continually assigned signals to find the proper ordering.
	
\item \textbf{Case 3}. $\mathtt{assign} ~~\mathrm{read\_data} = \mathrm{read\_data} ~\&~ \mathrm{content};$
	
There is a circular dependency between the left- and right-hand side of the
assignment.	Circular dependencies involving only combinational logic are caught during a step of preprocessing and
are out of scope. Running Sylvia with the ``-G'' flag enabled will output a
dataflow graph and inform users of combinational loops present in their
designs.
\end{enumerate}

%%  \cks{I thought we might want some pseudo code explaining this, but it got too
%%    complicated}
   
%%  \begin{figure}[h]
%%    \centering
%%    \begin{framed}
%%      \begin{lstlisting}[style={C-style}]
%% //Preprocessing
%% if (combinational_loops_present())
%%   return;

%% //Symbolic execution
%% A /*ordered list of always blocks in module*/
%% C /*ordered list of continuously assigned
%%   signals in module*/
%% for a in A:
%%   symbolically_explore(a); //track all signals that are updated
%%        \end{lstlisting}
%%    \end{framed}
%%    \caption{Algorithm for handling continuous assignments}
%%    \label{lst:algorithm}
%%    \end{figure}
       
Having considered the four cases, we can describe the algorithm for handling
continuous assignments within a module. First, check for any combinational loops
during preprocessing. If present,
Sylvia cannot proceed. Otherwise, during symbolic execution of a module, Sylvia first
computes the ordered list of $\mathtt{always}$ blocks in the module and the ordered list of
continuously assigned signals in the module, each ordered by dependency. Then Sylvia symbolically evaluates
each $\mathtt{assign}$, in order. Then, Sylvia
symbolically executes each $\mathtt{always}$ block. As the block is executed Sylvia keeps track of a dirty bit for each signal, which gets set to 1 when the
signal is updated. Once a single $\mathtt{always}$ block has been symbolically executed, Sylvia re-evaluates
every $\mathtt{assign}$ statement, in order, for which the right-hand side involves a dirty
signal. During this 
re-evaluation, Sylvia continues to track when signals become dirty. Finally,
Sylvia moves on to symbolically execute the next $\mathtt{always}$ block.
 
%% If a continuous assignment is present within a module, after the exploration of an always block, the symbolic execution engine recompute wires when \textit{signals on which they depended on} got updated in order to keep the internal state consistent. The Execution Manager keeps track of a dirty bit for each signal, that gets set to 1 when when it gets written to. Then at the end of the always block, we are able to use the signals that have been updated as a mask into our dependences to figure out which values need to be recomputed. 



\subsubsection{Conditional Expressions}
\label{sec:conditionalaexpressions}
Conditional expressions in Verilog are expressed syntactically using the traditional ternary operator, where you have 3 expressions (however, they can be nested), with the first being a boolean expression. We have an example of a non-nested conditional expression on line 24 of Figure 1. Sylvia offers two modes of execution for handling these constructions, as there are tradeoffs associated with both options. The choice is ultimately left up to the user.

 One option is for conditional expressions to be handled as control flow structures, meaning each decision point or boolean condition within a conditional expression will be allocated a bit in the \textit{pathcode}. This also means that the conditions appearing in the predicate will appear in the path condition. For some designs that might include deeply nested conditional expressions, and may incur an exponential increase in the complexity of the search space. 

The alternative is that the update is only seen in the symbolic store, not in
the path condition. This means the signal whose right-hand side was a
conditional expression would get a new symbolic expression in the symbolic store
that is of the form:
\begin{gather}
 \texttt{If(cond, symbolic\_store[\ true\_expr]\ } \\
     \texttt{symbolic\_store[\ false\_expr]\ )}
\end{gather}

This would then need to be properly parsed and loaded into the Z3 solver as an ITE query. These symbolic expressions can get messy and complex very quickly. 

%At the end of every clock cycle, we perform a simplification pass to see if these conditional symbolic expressions can be simplified before being sent to the Z3 solver. For example, if the condition in the predicate is false given some information available to us in the path condition or symbolic store, we can collapse the conditional expression down to a simpler form. 

\subsubsection{Non-blocking Assignments} 
\label{sec:nonblockingassigns}
A third challenge is parallelism is present within and across always blocks. So in Figure~\ref{lst:queuemodule}, all of the statements on lines 14-20 will be will be executed in parallel every time the clock signal goes high. First, we need to ensure clock-cycle accuracy of the state updates, or that statements actually look like they executed in parallel when an observer inspects the symbolic store. 

Second, it would be a naive approach to consider a symbolic execution tree that considered all possible orderings of these possible statements, even though all possible orderings of these statements are completely valid configurations of the design. We use a strategy akin to partial ordering reduction in model checking to reduce our total search space. Partial ordering reduction in model checking harnesses the commutative properties of concurrently executed transitions in systems that result in the same resultant states when executed in different orders \cite{Flanagan2005reduction}. In our case, these statements will result in the same symbolic state explored in different orders, so can just choose one to reduce the search space. 

To summarize, the key takeaway is once we've picked an ordering, parallel statements explored individually by the engine need to appear as if they were symbolically executed in parallel. The symbolic execution engine is visiting each statement one by one and updating the store one by one, but at the end of each clock cycle, the internal state must be clock-cycle accurate. Sylvia maintains this by storing the previous value of registers at the beginning of the new clock cycle. When an always block is being explored, any reads need to come from the previous values that we just stored prior to beginning execution. This ensures that no matter what order we decide to explore the statements in, the resultant state at the end of the block is consistent at the next clock-cycle boundary. 

\subsubsection{Hierarchical Modules}
\label{sec:hierarchicalmodules}


So far, we have considered the issues of continuous assignments and non-blocking assignments
within a single module. However, hardware designs are modular and hierarchical in nature. Any
individual module may instantiate an arbitrary number of submodules, which may
depend on each other in unknown ways. Consider the schematic of a design shown
in Figure~\ref{fig:twoqueueschematic}, in which a top module instantiates two
submodules, mod1 and mod2. The output of mod1 becomes the input to mod2, after
first passing through some combinational logic, shown in the Figure as a
circle. For example, the output may be partially masked before it is fed into
mod2. Similarly, the output of mod2 becomes the input to mod1. The signals
connecting the two submodules are defined in the top-level module. If, during
the symbolic execution of mod1, the output signal is updated, that needs to be
reflected in the top-level module.
% \cks{I think the queue example is good, but I
%  also think a figure is helpful. I don't know, they are both here and we can
%  decide!}  commenting out for now!
  
The queue example in Figures~\ref{lst:twoqueuestop} and \ref{lst:queuemodule} provides a
concrete example. In Figure~\ref{lst:twoqueuestop}, the $\mathtt{top}$ module instantiates
two queue modules, q1 and q2. The
signals of interest to us here are $\mathtt{data}$ and
$\mathtt{read\_data}$. The first, $\mathtt{data}$ is used by q1 as the output signal
$\mathtt{read\_data}$. In the body of q1 (Figure~ref{lst:queuemodule}), let's assume $\mathtt{read\_en}$ is
true and $\mathtt{read\_data}$ gets updated on line 24 through a continuous
assignment. Now from the top level module's view, the $\mathtt{data}$ wire
should have the updated value. And this updated value should be reflected in $\mathtt{data}$ before Sylvia
starts symbolic exploration of q2, where it is used as the input signal
$\mathtt{write\_data}$. 

%\cks{A piece, I don't quite get -- does it matter that
%the assignment to read\_data was continuous? Either way, Sylvia has to do the
%recomputation of parameter--argument pairs, right?} 
%\kar{This is correct, and now 
%I'm remembering why I had put this in the hierarchical submodules section originally I think. If read\_data was 
%given the value of contents directly in the always block it would be the same thing. I really think the only challenge 
%with hierarchical modules is the tracking of inter-modular dependencies. I might add that back and see?}


\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth,trim=.5in 2in 4.5in 1in,
    clip]{figures/twoqueueschematic}
  \caption{A simplified schematic with inter-module continuous assignments.}
  \label{fig:twoqueueschematic}
  \end{figure}
    

The algorithm for handling inter-module continuous assignments and is similar to
that for intra-module continuous assignments, but
with inter-module dependencies taken into consideration. At the end of each
exploration of a submodule,
Sylvia takes a pass to recompute and synchronize all parameter and argument
pairs where the parameter is an internal wire or register from the parent and
the argument is an output of the submodule.


%% discussed in section 3.3.3. 

%% The presence of hierarchical submodules also presents a challenge when it comes to continuous assignments, too. We previously stated that we make the assumption that input signals being fed into a module are fixed for that clock cycle. However, if a top level or enclosing module instantiates a submodule and feeds in some internal signals as inputs, any changes to these signals incurred in the submodule through assignment statements need to be propagated back up and reflected in the top-level module.

%% We will revisit the queue example to explain Sylvia's solution to handling this,
%% referencing the top level module in Figure 2 to get an idea of how Sylvia
%% operates across modules. So in Figure 2, we instantiate a queue module, q1. The
%% signals of interest to us here are data and read\_data. Data is being fed q1 as
%% the value for read\_data. Then if we look in Figure 1, let's assume read\_en is
%% true and we update read\_data on line 24 to get the value of content. Now from
%% the top level module's view, the data wire should be holding content. 

%% The implementation strategy is similar to that for continuous assignments, but now the dependencies we are tracking with the Execution Manager are inter-modular dependencies. At the end of each exploration of a child module, Sylvia takes a pass to recompute and synchronize all parameter and argument pairs where the parameter is some internal wire or register from the parent and the argument is an output of the submodule. 

\subsubsection{Multiple Clock Cycles}
\label{sec:multipleclockcycles}As mentioned in the background section, the symbolic execution of a hardware design means that symbolic exploration of design for one clock tick produces a tree where the root node represents the design in the reset set or initial state, and each each leaf node corresponds to a ``next-state'' for execution to begin with on the rising edge of the next clock cycle. To explore a design for two clock cycles would mean exploring the design again starting from each leaf node of the tree we constructed during clock cycle 0. Allowing for multi-clock cycle path means an explosion in complexity of the search space, however, it is important for applicability to real systems. For example, pipelined CPUs may have security vulnerabilities residing in the last stage of the pipeline, so Sylvia would need to run for at least the number of pipeline stages in order for the signals to propagate to through the whole pipeline and find the assertion violation. For a design like an AES module, we want to run exploration for as many cycles as there are ``rounds.'' 
    
 At the end of each traversal, there is a state merging step, where all of inputs and wires get fresh symbols for the next cycle while stateful elements carry over their expressions from the previous cycle. As we explore the design, we keep a cache of the states we've seen stored by the specific module and \textit{pathcode} pairing.  This caching of ``seen states'' will be useful for the optimizations described in section 3.7. 
 
 \subsection{Optimizations}
 \label{sec:optimizations}
The final phase of Sylvia includes several optimizations for producing assertion violations. Note that these are strategies that are made possible by our development of a hardware-oriented symbolic execution engine. Working within other software-oriented tools, like KLEE, leaves us with little control over how to explore the design and no space to experiment with hardware specific search techniques. Hardware designs contain large amounts of concurrency not present in software programs which are largely sequential in execution. For example, we may have parallel always blocks within modules that are executing at the same time or different modules that all execute in lock-step at the positive edge of a clock. This parallelism present in hardware allows for targeted searches and optimizations during Sylvia's exploration that we use to help mitigate the path explosion problem and increase performance. 

In this section we will discuss three different optimizations Sylvia implements for improving the performance and decreasing the time needed to find security assertion violations.

 \subsubsection{Redundant Submodules}. 
 \label{sec:redundantmodules}
 As mentioned in the preprocessing section, when hierarchical modules are dependent on each other, we are faced with the challenge of figuring out the correct ordering for exploration.  However, when the modules are independent or even duplicate instantiations of the same module there is room for reduction in the total search space. 
 
 Take a simple processor, for example, that might have memory, ALU and decoder submodules. There might be 20 paths through the memory, 10 paths through the ALU
and 2 paths through the decoder, but all the paths start from a single root in the top-level module. Some of the sub-paths may be completely disjoint in terms of the signals they involve and some may not. This means that some of the time
we will need to perform a serialization and impose an order in order to first
 resolve required dependencies, as discussed previously in section 3.1.4,  but
sometimes this may be unnecessary and submodules could be symbolically executed
independently of each other. This is an opportunity for optimization in the case when there are redundant submodule instantiations. The main idea of the optimization is that we explore the redundant submodule once for each path. Then instead of re-exploring again for each duplicate module, we can statically merge in the symbolic store and path condition for the given \textit{pathcode}. 
 
% We will refer to a pairing of a symbolic store and a path condition as a state. The way we do the merging is by choosing one state to be the resultant state, with the other state getting merged into it. When merging two states there are two possibilities for each signal that is part of the merge: the signal is unique to one of the two states, or it is common between them. In the resultant state, we first bring in all the unique signal name-value pairs from the second state. Then for all the signals that are common between both blocks, if any of the unique/ newly merged symbols are dependent on this signal, we would need to replace those symbols with the one from the resultant state.  The constraints in the path condition of the state being merged in undergoes the same dependency aware symbol substitution. Once the symbols are substituted, the new constraints are pushed to the resultant path condition. So long as there is no contradiction in the constraints, the states have been merged.  %\kar{this is not well-explained, try again more concisely}

 \subsubsection{Cone of Influence Analysis}. 
  \label{sec:coianalysis}
 This optimization performs pruning of the state space at the block level. The general idea is that Sylvia will read in the expressions supplied in the security assertions, performs some dependency analysis over the signals in the assertions and then complete an AST traversal to determine which blocks contain information about the signals of interest or their dependencies. In particular, a mapping is constructed between always blocks and security critical signals, so that each always block may have a subset of security critical signals associated with it. Sylvia always reads the assertions in at the top level module, so we will know exactly what signals are of interest to us as we begin exploration of the design.  After this initial pass, we only explore the blocks that have a non-empty set of signals associated with them in the final mapping.
 
  \subsubsection{Parallel Always Blocks}. 
   \label{sec:parallelblocks}
  Two always blocks are parallel if their sensitivity lists overlap, meaning that given some signal in the list goes high, both blocks of statements are executed in parallel. The key insight of this optimization is that if we can determine independence between two always blocks, then we shouldn't need to explore all orderings of blocks relative to one another. Instead, we can explore each always block independently, statically merging together the states and path conditions for a given \textit{pathcode}.  This optimization ends up being relatively straightforward because we make an assumption of no race conditions. Sylvia applies the optimization assuming the design has no race conditions, but will output a warning if it detects that there is race condition across two always blocks. A race condition is the result of a single signal appearing on the left-hand side of more than one non-blocking assignment within more than one parallel always block in a given clock tick. While you can imagine a good hardware engineer would avoid doing this, it is indeed legal Verilog to do so. When this does happen, per the official Verilog standard, the last nonblocking assignment wins. The assignment within the always block that appears later in the code will be the one that takes effect \cite{verilog}. 
  
  
% Additional Comments
%Verilog supported
%
%Sylvia can handle Verilog written to the IEEE Std 1364-2005.  Sylvia is not strictly operating over the synthesizeable subset -- Sylvia supports the initial statement -- and this is where we insert our own macros for handling assertions.
%
%Wrong claim end of 2.
%
%We will soften our wording of this claim. There are structural differences between hardware and software, leading to different trade-offs to be made, not to an easier verification problem.



